A matrix-free isogeometric Galerkin method for Karhunen-Lo\`eve approximation of random fields using tensor product splines, tensor contraction and interpolation based quadrature

The Karhunen-Lo\`eve series expansion (KLE) decomposes a stochastic process into an infinite series of pairwise uncorrelated random variables and pairwise $L^2$-orthogonal functions. For any given truncation order of the infinite series the basis is optimal in the sense that the total mean squared error is minimized. The orthogonal basis functions are determined as the solution of an eigenvalue problem corresponding to the homogeneous Fredholm integral equation of the second kind, which is computationally challenging for several reasons. Firstly, a Galerkin discretization requires numerical integration over a $2d$ dimensional domain, where $d$, in this work, denotes the spatial dimension. Secondly, the main system matrix of the discretized weak-form is dense. Consequently, the computational complexity of classical finite element formation and assembly procedures as well as the memory requirements of direct solution techniques become quickly computationally intractable with increasing polynomial degree, number of elements and degrees of freedom. The objective of this work is to significantly reduce several of the computational bottlenecks associated with numerical solution of the KLE. We present a matrix-free solution strategy, which is embarrassingly parallel and scales favorably with problem size and polynomial degree. Our approach is based on (1) an interpolation based quadrature that minimizes the required number of quadrature points; (2) an inexpensive reformulation of the generalized eigenvalue problem into a standard eigenvalue problem; and (3) a matrix-free and parallel matrix-vector product for iterative eigenvalue solvers. Two higher-order three-dimensional benchmarks illustrate exceptional computational performance combined with high accuracy and robustness.

==> settings/mycommands.tex <==
%% Abkürzungen
\newcommand{\NYS}{Nystr{\"o}m\xspace}
\newcommand{\BEZ}{B{\'e}zier\xspace}
\newcommand{\Lame}{Lam{\'e}\xspace} % Lame


%% Format of vectors, matrices and spaces
\newcommand{\myMat}[1]{\mathbf{#1}}
\newcommand{\mySpace}[1]{\mathcal{#1}}
\newcommand{\myVec}[1]{\mathbf{#1}}
\newcommand{\myVecGreek}[1]{\boldsymbol{#1}}
\newcommand{\myNorm}[1]{\lVert #1 \rVert}
\newcommand{\myCardinality}[1]{\# #1}

%% general indices
\newcommand\indexA{i} 		% first normal index
\newcommand\totalA{I} 		% total number of elements of index A
\newcommand\indexB{j} 		% second normal index
\newcommand\totalB{J} 		% total number of elements of index B
\newcommand\indexC{k} 		% third normal index
\newcommand\totalC{K} 		% total number of elements of index C
\newcommand\indexD{m} 		% forth normal index
\newcommand\totalD{M} 		% total number of elements of index D
\newcommand\indexE{n} 		% forth normal index
\newcommand\totalE{N} 		% total number of elements of index E
\newcommand\indexF{t} 		% forth normal index
\newcommand\totalF{T} 		% total number of elements of index F
\newcommand\indexG{l} 		% forth normal index
% \newcommand\indexG{\ell} 		% forth normal index
\newcommand\totalG{L} 		% total number of elements of index G

%% specifiv indices
% \newcommand\indexGauss{g}
% \newcommand\totalGauss{n}
\newcommand\indexGauss{q}
\newcommand\totalGauss{Q}
\newcommand\indexSpan{s}	% index of span of B-spline segment
\newcommand\indexSpanTrimmed{t}	% index of trimmed span of B-spline segment
\newcommand{\indexLevel}{\ell}	% index for the refinement level
\newcommand{\totalLevel}{L}	% index for the refinement level


%% multi index
\newcommand\mIndexI{\myVec{i}}
\newcommand\mIndexJ{\myVec{j}}
\newcommand\mIndexP{\myVec{p}}
% \newcommand\mIndexA{\myVec{i}} 	% multi index
% \newcommand\mTotalA{\myMat{I}} 	% multi index
% \newcommand\mIndexB{\myVec{j}} 	% multi index
% \newcommand\mIndexP{\myVec{p}}	% multi index


%% NURBS 
\newcommand{\Bspline}{B} 		% symbol for B-spline
\newcommand{\BsplineSeg}{\mathcal{B}} 	% symbol for B-spline segment
% \newcommand{\BsplineSeg}{S}} 	% symbol for B-spline segment
\newcommand{\NURBS}{R} 			% symbol for NURBS
\newcommand{\KV}{\varXi} 		% knot vector
\newcommand{\KVRefined}{\hat{\varXi}} 	% knot vector refined
\newcommand{\KVC}{\varLambda} 		% knot vector of the Cauchy data - nystroem
\newcommand\uu{\xi} 			% Local NURBS coordinates
\newcommand\uuRefined{\hat{\uu}} 	% inserted knots
\newcommand\vv{\uu} 			% Local NURBS coordinates
\newcommand\UVsurf{\pt{\uu}} 	% Local NURBS coordinates
\newcommand\uusurf{\uu_1} 		% Local NURBS coordinates
\newcommand\vvsurf{\vv_2} 		% Local NURBS coordinates
\newcommand\uuc{a} 			% Local NURBS coordinates for artificial knot vector  of the Cauchy data
\newcommand\multi{m} 			% Multiplicity of a knot
% \newcommand{\w}{w} 			% symbol for the NURBS weights
% \newcommand{\W}{\w(\uu)} 		% symbol for NURBS weighting function
\newcommand{\knotinsertion}{d_k}

\newcommand\refElXi{r}                  % coordinates of the reference element

%% point types
\newcommand{\CP}{\pt{c}}		% control points
\newcommand{\CPRefined}{\hat{\CP}} 	% refined control point
\newcommand{\CPara}{c}			% control parameter
\newcommand{\CPH}{\CP^h} 		% homogeneous control point
\newcommand{\CPHRefined}{\hat{\CP}^h} 	% homogeneous control point
\newcommand{\CPCoons}{\CP^{\uu}}	% control points for local Coons patch
\newcommand\collocationPoint{\pt{x}^c}	% collocation point
\newcommand\collocationPointNys{\collocationPoint}	% collocation point
\newcommand{\GP}{\pt{y}} 		% quadrature point

%% abscissa
\newcommand\abscissa{\bar{\uu}}			% abscissa
\newcommand\abscissaAnyDim{\bar{\pt{\uu}}}	% abscissa general dimension
\newcommand\greville{\abscissa}		% Greville abscissa
% \newcommand\greville{\abscissa^g}		% Greville abscissa
\newcommand\grevilleAnyDim{\bar{\pt{\uu}}^g}	% Greville abscissa general dimension
\newcommand\demko{\abscissa^d}		% Demko abscissa
\newcommand\uuExtended{\abscissa^e}	% Local NURBS coordinates and Greville
\newcommand\abscissaShift{\alpha}	% offset for discontinuous basis functions (2-ring)
% \newcommand{\discontinuousShift}{\hat{\alpha}} % shift of abscissa (not 2-ring approach)
\newcommand\collocP{\bar{\uu}^c}	% symbol for collocation points

%% spaces
\newcommand{\BsplineSpace}{\mathbb{S}} % symbol for B-spline space
\newcommand{\ApproxSpace}{\mathbb{S}_h}% symbol for B-spline space
\newcommand{\SolutionSpace}{\mathbb{S}} % symbol for B-spline space

%% degrees and order
\newcommand\pu{p}			% NURBS degree on u
\newcommand\polyorder{\tilde{\pu}}	% polynomial order on u
\newcommand\pv{p_{v}}			% NURBS degree on v
\newcommand\puc{p_{q}}			% nystroem quadratur order on u
\newcommand\puCauchy{\pu_c}		% degree of Cauchy data basis
\newcommand\puGeo{\pu_g}		% degree of Geometry basis
\newcommand\pusurf{\pu_1} 		% Local NURBS degree
\newcommand\pvsurf{\pu_2} 		% Local NURBS degree

%% patch types
% \newcommand{\curve}{\pt{x}\operate{\uu}}
\newcommand{\curve}{\pt{C}}
% \newcommand{\curve}{{\tau}}
% \newcommand{\curveRefined}{\hat{\pt{x}}\operate{\uu}}
% \newcommand{\curveRefined}{\hat{\pt{x}}}
\newcommand{\curveRefined}{\hat{\curve}}
% \newcommand{\curveBez}{\pt{x}_{b}}%%\operate{\xi_1}}
\newcommand{\curveBez}{{\tau}_{b}}%%\operate{\xi_1}}
% \newcommand{\curveBezOpposite}{\pt{x}_{e}}%%\operate{\xi_1}}
\newcommand{\curveBezOpposite}{{\tau}_{e}}%%\operate{\xi_1}}

%% element types
\newcommand\gradingSubEl{\ell} 		% # of sub-elements introduced by grading
% \newcommand\be{\omega} 			% boundary element (NURBS)
\newcommand\be{\gamma} 			% boundary element (NURBS)
% \newcommand{\IGAel}{e_\uu} 		% integration element
\newcommand\ieKs{\tau} 		% non-zero knot span
\newcommand\ieLocal{\tilde{\ieKs}} 		% local integration element for EXTENDED B-splines
% \newcommand\ieg{\tilde{\ieKs}} 		% Element for Gauss integration
% \newcommand\iegLocal{\grave{\ieKs}} 	% Local element for Gauss integration
\newcommand\ieReference{\grave{\ieKs}} % reference element [-1,1]

% \newcommand\ieKs{\tau^{\emptyset}} % non-zero knot span
% \newcommand\ieAr{\tau^{\boxtimes}} % integration region with aspect ratio 1
% \newcommand\ie{\tau^{\boxplus}} % sub-element of hierarchically refined%

% \newcommand\ieKs{\tau^{\square}} % non-zero knot span
% \newcommand\ieAr{\tau^{\boxplus}} % integration region with aspect ratio 1
% \newcommand\ie{\tau^{\boxdot}} % sub-element of hierarchically refined

% \newcommand\ieAr{\hat{\tau}^{\boxplus}} % integration region with aspect ratio 1
% \newcommand\ie{\hat{\tau}^{\boxdot}} % sub-element of hierarchically refined
%\newcommand\ie{\hat{\tau}^{\boxdot}} % sub-element of hierarchically refined




%% Extended B-splines
\newcommand{\exBspline}{B^e} 		% symbol for extended B-spline
\newcommand{\degSet}{\mathbb{J}} 	% symbol for the set of degenerated B-splines
% \newcommand{\degSet}{\eta} 	% symbol for the set of degenerated B-splines
\newcommand{\innerSet}{\mathbb{I}} 	% symbol for the set of degenerated B-splines
\newcommand{\exteriorSet}{\mathbb{K}} 	% symbol for the set of degenerated B-splines
\newcommand{\NSet}{\mathbb{T}} 	  	% symbol for the set of knot Menge for Nbasis
\newcommand{\eweight}{e} 	  	% symbol for the extrapolation weight
\newcommand{\Nbasis}{\psi} 	  	% symbol for newton's basis
\newcommand{\taylorpoint}{\tilde{\uu}} % extension point for taylor expansion
% \newcommand{\poly}{\gamma} 		% factor of a polynomial: \poly_1 * x + \poly_2 
\newcommand{\poly}{{\alpha}} 		% factor of a polynomial: \poly_1 * x + \poly_2 
\newcommand{\lambdapoint}{\mu} 	% extension point for deBoorFix functional
% \newcommand{\lambdapoint}{\upsilon} 	% extension point for deBoorFix functional
\newcommand{\trim}{t}
\newcommand{\variableKnot}{\hat{\uu}}

%% Extended THB-splines
\newcommand{\refinementCriterion}{c_e}  % symbol for the refinement criterion which determines the extrapolation length
\newcommand{\extrapolationLength}{d_e}
\newcommand{\knotSpanSize}{h_{\uu}}
\newcommand{\refinementLevel}{\ell}
\newcommand{\abscissaFineScale}{\abscissa^{(\refinementLevel+1)}}
\newcommand{\subCoef}{\alpha}


%% independent field approximation 
\newcommand{\GeoBasis}{\theta} 		% basis funtion related to the geometry field
% \newcommand{\PrimaryBasis}{\varphi} 	% basis funtion related to the primary field
% \newcommand{\DualBasis}{\psi} 		% basis funtion related to the dual field
\newcommand{\PrimaryBasis}{\Bspline^{\primary}} 	% basis funtion related to the primary field
\newcommand{\DualBasis}{\Bspline^{\dual}} 		% basis funtion related to the dual field
\newcommand{\sub}{s} 		%% sub-indices for sub-parametric formulations
\newcommand{\iso}{i} 		%% sub-indices iso-parametric formulations



%% Nyström
\newcommand{\LCNadmissibility}{\eta} 	% symbol for local correction admissibility factor
\newcommand{\LCNarea}{\Omega_{\collocationPointNys}}



%% local refinement
\newcommand{\locRefInfo}{\grave{\pt{\uu}}} % point for local refinement
\newcommand{\transMatrix}{\mathbf{T}}
\newcommand{\nodeMatrix}{\mathbf{N}}
\newcommand{\nodeMatrixLocal}{\nodeMatrix^{\ell}}
\newcommand\Lieg{l} 
\newcommand\LiegLocal{l}



%% analysis stuff
% \newcommand{\hoelder}{\gamma} 		% Hölder constant
\newcommand{\hoelder}{\upsilon} 		% Hölder constant
\newcommand{\DOF}{n} 			% symbol for degrees of freedom
\newcommand\cdim{d}			% Cartesian dimension
\newcommand\KVdim{\delta}			% Cartesian dimension
\newcommand{\domain}{\Omega}
% \newcommand{\patchdomain}{\Omega^{\textnormal{v}}}
\newcommand{\patchdomain}{\mathcal{A}^{\textnormal{v}}}
% \newcommand{\patchdomain}{\Gamma_{\textnormal{v}}}
\newcommand{\boundary}{\Gamma}
\newcommand{\boundaryNonSmooth}{\boundary^0}
\newcommand{\Ltwo}{L_{2}}
\newcommand{\GramDet}{G}
\newcommand\primary{u} 			% primary variable - displacements in elasticity
\newcommand\primaryApprox {\primary_h} % primary variable - displacements in elasticity
\newcommand\dual{t} 			% dual variable - tractions in elasticity
\newcommand\utens{\primary} 		% displacement tensor field
\newcommand\ttens{\dual} 		% surface traction tensor
\newcommand\conductivity {k} 		% conductivity
\newcommand\uvek{\myVec{u}} 		% displacement vector field
\newcommand\tvek{\myVec{t}} 		% surface traction
\newcommand\uvekc{\tilde{\uvek}} 	% displacement vector at control points
\newcommand\tvekc{\tilde{\tvek}} %	 traction at control points


\newcommand{\LshapeCoord}{\zeta} 		% symbol for degrees of freedom

%% Real numbers
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}

%% mappings
\newcommand{\perspectiveMap}{\op{P}}

%% math operators
\DeclareMathOperator{\sgn}{sgn}
% \DeclareMathOperator{\dx}{d}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\troot}{root}
\DeclareMathOperator{\dist}{\mathrm{dist}}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\diag}{diag}

%% Integral Operator
\newcommand\op[1]{\mathcal{#1}}
\newcommand\operate[1]{(#1)}
\newcommand\dx[1]{\;\text{d}#1}

%% H-matrices
\newcommand{\rk}{\mathcal{R}_k} % Low Rank Matrices
\newcommand{\h}{\mathcal{H}} % Hierarchical
\newcommand{\hmatrix}{\mbox{$\h$-matrix}\xspace}
\newcommand{\hmatrices}{\mbox{$\h$-matrices}\xspace}
% \newcommand{\rkm}{\rk-} % Low Rank Matrices
\newcommand{\orderof}[1]{\mathcal{O}\left(#1\right)} % Landau Symbol
% \newcommand{\storage}[1]{\mathsf{St}\left(#1\right)} % Storage
% \newcommand{\operations}[2]{\mathsf{Op}_{\mathit{#1}}\left(#2\right)}
% Operations
\newcommand{\order}{\mathcal{O}} % Landau Symbol only
\newcommand{\storage}{\mathsf{St}} % Storage 
\newcommand{\operations}{\mathsf{Op}} % Operations



%% URLs
\providecommand\url[1]{\emph{#1}}
% \newcommand\url[1]{\emph{#1}}


%% Signum-function
%\newcommand\sig[1]{\operatorname{sign} \left( #1 \right)} 



%% Integrals with any sign in the middle
%% (see Latex Symbels AMS p105.
\newcommand\Xint[1]{\mathchoice {\XXint\displaystyle\textstyle{#1}}%
  {\XXint\textstyle\scriptstyle{#1}}%
  {\XXint\scriptstyle\scriptscriptstyle{#1}}%
  {\XXint\scriptscriptstyle\scriptscriptstyle{#1}}%
  \!\int}
\newcommand\XXint[3]{{\setbox0=\hbox{$#1{#2#3}{\int}$}
    \vcenter{\hbox{$#2#3$}}\kern-.5\wd0}}
%\newcommand\ddashint{\Xint{=}} %% dashed integral
\newcommand\dashint{\Xint{-}} %% double sashed integral


%\newcommand\cpvint{-\!\!\!\!\!\!\!\!\!\int}
%\newcommand\cpvint{\dashint}
\newcommand\cpvint{\Xint{c}}
%\newcommand\cpvint{\strokedint}

\newcommand\mymin[1]{\min\{#1\}}
\newcommand\mymax[1]{\max\{#1\}}
\newcommand\fromto[2]{\{ #1, \dots, #2 \}}
\newcommand\mal{\cdot}




%% Differential Operators
\renewcommand{\div}{\nabla \cdot}
\newcommand{\grad}{\nabla}
\newcommand{\curl}{\nabla \times}
\newcommand{\Laplace}{\Delta}
\newcommand{\dTr}{\op{T}} %% conormal derivative

\newcommand\dgamma[1]{\dx\mathrm{s}_{\pt{#1}}}
\newcommand\domega[1]{\dx{\pt{#1}}}


%\newcommand{\Tr}{\mathrm{Tr}} %% boundary trace
% \newcommand{\dTr}{\op{T}} %% conormal derivative

%% Vector and matrix notation
% \newcommand\vek[1]{\mathbf{#1}}
% \newcommand\veks[1]{\boldsymbol{#1}}
% \newcommand\mat[1]{\mathbf{#1}}
\newcommand\tens[2]{\mathsf{#1}}
% 
\newcommand{\trans}{\intercal} % transposed matrix/vector
\newcommand{\inv}{{-1}} % inverted matrix

%% Abbreviations



\newcommand\ct{T} % cluster tree
\newcommand\bct{T_{I\times J}} % block cluster tree

%\newcommand\fund[3]{\tens{#1}{#2}{][
\newcommand\fund[1]{\tens{#1}{2}}
% \newcommand\fund[2]{\tens{#1}{2}{\ofpt{#2}}}
% \newcommand\fund[3]{\tens{#1}{2}\left(\pt{#2},\pt{#3})}

\newcommand\dirac{\delta}
\newcommand\kronecker{\delta}





%% Text in math
\newcommand\beistrich{,\,}
%\newcommand\with{\quad\text{with}\,}
\newcommand\und{\,\text{and}\,}
\newcommand\oder{\,\text{or}\,}
\newcommand\with{\,\text{with}\,}
\newcommand\for{\,\text{for}\,}
\newcommand\where{\,\text{where}\,}

%% Points
% \newcommand\pt[1]{\veks{#1}}
% \newcommand\pt[1]{\myVec{#1}}
\newcommand\pt[1]{\boldsymbol{#1}}
\newcommand\ofpt[1]{(\pt{#1})}
% \newcommand\ofpt[1]{(\pt{#1})}
\newcommand\sourcept{\tilde{\pt{x}}}
\newcommand\fieldpt{\hat{\pt{x}}}
\newcommand\boundarypt{\pt{y}}


%% Symbols
\newcommand\eps{\varepsilon}
\newcommand\err{\epsilon}
\newcommand\residual{\err}
\newcommand\mychi{\mathcal{X}}

%% Todo-list
\newcommand\done{\checkmark}

%% Figures
\newcommand{\myfig}[4]{
  % file=#1, size=#2, caption=#3, label=#4
  \begin{figure}[ht]%[htb!]
    \centering
    \includegraphics[width=#2]{#1}
    \caption{#3}
    \label{fig:#4}
  \end{figure}
}


\ifdefined\tikzSubmission
%% TikZ Figure with relative scaling to full linewidth (tikzscale-package)
\newcommand{\tikzfig}[5]{
  % file=#1, size=#2, caption=#3, label=#4, figno=#5
%   \begin{figure}[ht]%[htb!]
    \centering
    \includegraphics{#5}
    \caption{#3}
    \label{fig:#4}
%   \end{figure}
}
\else
%% TikZ Figure with absolute scaling
\newcommand{\tikzfig}[5]{
  % file=#1, size=#2, caption=#3, label=#4, figno=#5
%   \begin{figure}[htb!]

    \def\tkzscale{#2}
    \def\dirtikz{tikz} % define tikz directory
    \def\dirdata{data} % define data directory
    \centering
    \tikzsetnextfilename{#5}
    \input{#1}
    \caption{#3}
    \label{#4}
%   \end{figure}
}
\fi

%% add Tikz Subfigure
\ifdefined\tikzSubmission
\newcommand{\tikzsubfig}[5]{
    % file=#1, size=#2, subcaption=#3, label=#4, figno=#5
    \centering
    \includegraphics{#5}%
    \subcaption{#3}
    \label{#4}
}
\else
\newcommand{\tikzsubfig}[5]{
  % file=#1, size=#2, subcaption=#3, label=#4, figno=#5

    \def\tkzscale{#2}
    \def\dirtikz{tikz} % define tikz directory
    \def\dirdata{data} % define data directory
    \centering
    \tikzsetnextfilename{#5}
    \input{#1}
    \subcaption{#3}
    \label{#4}
}
\fi


%% Tables
\newenvironment{mytable}[4]%
{
  % #1=position #2=caption #3=label #4=table layout
  \begin{table}[#1]%[htb!]
    % \caption{#1}
    % \label{tab:#2}
    \def\mycap{#2}
    \def\mylabel{#3}
    \centering
    \begin{tabular}{#4}
      \toprule
%       #4 \\ 
%       \midrule
%       \hline%\noalign{\smallskip}
}
{
  %\noalign{\smallskip}
%   \hline
  \bottomrule
  \end{tabular}
  \caption{\mycap}
  \label{\mylabel}
  \end{table}
}
\newcommand{\mytableheader}[1]{
  % #1=header without line breaks (i.e. ' 1.col & 2.col & 3.col ' )
       #1 \\ \midrule
}

\newenvironment{mytableposition}[4]%
{
  % #1=caption #2=label #3=table layout #4=position
  \begin{table}[#4]%[htb!]
    % \caption{#1}
    % \label{tab:#2}
    \def\mycap{#1}
    \def\mylabel{tab:#2}
    \centering
    \begin{tabular}{#3}
      \toprule
%       #4 \\ 
%       \midrule
%       \hline%\noalign{\smallskip}
}
{
  %\noalign{\smallskip}
%   \hline
  \bottomrule
  \end{tabular}
  \caption{\mycap}
  \label{\mylabel}
  \end{table}
}
% \newcommand{\mytableheader}[1]{
%   % #1=header without line breaks (i.e. ' 1.col & 2.col & 3.col ' )
%        #1 \\ \midrule
% }






%% Algorithms
% % Algorithm comment style
% \newcommand{\store}{=} 	% symbol for storing with in algorithm
% \newcommand{\myinsert}{\leftarrow} 	% symbol for insertions with in algorithm
% % \renewcommand{\algorithmiccomment}[1]{\hspace{1cm} // #1} 
% \renewcommand{\algorithmiccomment}[1]{\hspace{1cm}$\vartriangleright$ #1} 
% % Algorithm environment
% \newenvironment{myalgorithm}[2]%
% {
%   % #1=caption #2=label
%   \begin{algorithm}
%     \caption{#1}
%     \label{#2}
%     \begin{algorithmic}[1]
% }   
% {
% \end{algorithmic}
% \end{algorithm}
% }

%% Todo-List
% \ifdefined\tikzSubmission
% \newcommand\todos[2]{ %
% }
% \else
% \newcommand\todos[2]{ %
% {
%   \ifdefined\tikzExtOn
%   \tikzset{external/export=false}
%   \fi
%   \todo[inline,size=\scriptsize,caption={List:
%     #1}]{ \begin{minipage}{\linewidth} #2 \end{minipage} } 
% }
% }
% \fi

% % Personalized comments
% \ifdefined\tikzSubmission
% \newcommand{\mycomment}[2][-]{ }%
% \else
% \newcommand{\mycomment}[2][-]{%
%   % initials of the author (optional) + note in the margin
%   {%
%     {
%     \ifdefined\tikzExtOn
%     \tikzset{external/export=false}
%     \fi
%     \setstretch{0.7}% spacing
%     \todo[color={green!33},size=\scriptsize]{
%       \textbf{[\uppercase{#1}]} #2}}%
%   }
% }%
% \fi


%% References to insert
% \ifdefined\tikzSubmission
% \newcommand{\todoref}[2][reference]{}
% \else
% \newcommand{\todoref}[2][reference]{%
%   {
%   \ifdefined\tikzExtOn
%   \tikzset{external/export=false}
%   \fi
%   \todo[color=blue!50,size=\scriptsize]{\emph{#2} #1}[{\color{blue!50}{\textsl{#2}}}]
% }
% }%
% \fi

\newcommand{\mychangeEq}[1]{\color{red}\textbf{#1}\color{black}}
% \newcommand{\mychangeEq}[1]{#1}
\newcommand{\mychange}[1]{\color{red}\textbf{#1}\color{black}\xspace}
% \newcommand{\mychange}[1]{\color{red}{#1}\color{black}\xspace}
% \newcommand{\mychange}[1]{\protect\hl{#1}}

\ifdefined\TodoNotes
    %%% Marked revisions and annotations
    \newcommand{\mycomment}[2][-] % works for okular too
    {
    %   \pdfcomment[color=yellow,voffset=3pt,opacity=0.75,author=#1]{#2}
%       \ignorespaces
        {%
            \ifdefined\tikzExtOn
            \tikzset{external/export=false}
            \fi
%             \setstretch{0.1}% spacing
            \todo[color={green!33}]{ \textbf{[\uppercase{#1}]} #2}
            \pdfcomment[color=yellow,opacity=0.0,author=#1]{}%% invisible comment to show comment in annotations list
        }%
    }	
    % \sethlcolor{green} % set highlight color to green
    \newcommand{\myhighlight}[2][-] % works for okular too
    {
    \pdfcomment[color=yellow,voffset=-5pt,hoffset=3pt,opacity=0.0,author=#1]{}%% invisible comment to show highlight in annotations list
    \hl{#2}%
    }	
    \setstcolor{red} % set strike out color to red
    \newcommand{\mydelete}[2][-] % works for okular too
    {
    \pdfcomment[color=yellow,voffset=-5pt,hoffset=3pt,opacity=0.0,author=#1]{}%% invisible comment to show highlight in annotations list
    \st{#2}%
    }
\else
    \newcommand{\mycomment}[2][-]{}
    \newcommand{\myhighlight}[2][-]{}
    \newcommand{\mydelete}[2][-]{}
\fi

\ifdefined\tikzSubmission
\newcommand\revdel[2]{}
\newcommand\revadd[2]{}
\newcommand\revmod[2]{}
\newcommand\revcomment[1]{} % for cases where pdfmarkupcomment does not work (i.e. figures)
\else
\newcommand\revdel[2]{ %
{
  \pdfmarkupcomment[markup=StrikeOut,color=red,author=Marussig and Zechner]{#1}{#2}
}
}
\newcommand\revadd[2]{ %
{
  \pdfmarkupcomment[markup=Underline,color=green,author=Marussig and Zechner]{#1}{#2}
}
}
\newcommand\revmod[2]{ %
{
  \pdfmarkupcomment[markup=Highlight,color=yellow,author=Marussig and Zechner]{#1}{#2}
}
}
\newcommand\revcomment[1]{ %
{
  \pdfcomment[color=yellow,author=Marussig and Zechner,voffset=8pt,opacity=0.8]{#1}
}
}
\fi




%% Theorems and remarks
% \theoremstyle{remark}
% \newtheorem*{remark}{Remark}
\newtheoremstyle{myremark}% ⟨name⟩ 
{3pt}% Space above
{3pt}% Space below
{}% Body font
{}% Indent amount
{\itshape}% Theorem head font
{:}% Punctuation after theorem head
{.5em}% Space after theorem head
{}% Theorem head spec (can be left empty, meaning ‘normal’)
\theoremstyle{myremark}
\newtheorem*{remark}{Remark}

%% References
\newcommand{\myEqref}[1]{Equation~(\ref{#1})}
\newcommand{\myeqref}[1]{equation~(\ref{#1})}	
\newcommand{\myfigref}[1]{Figure~\ref{#1}}
\newcommand{\myFigref}[1]{Figure~\ref{#1}}
\newcommand{\myRef}[1]{(\ref{#1})}
\newcommand{\mytabref}[1]{Table~\ref{#1}}
\newcommand{\myTabref}[1]{Table~\ref{#1}}
\newcommand{\mySecref}[1]{Section~\ref{#1}}
\newcommand{\mysecref}[1]{Section~\ref{#1}}
\newcommand{\myalgref}[1]{Algorithm~\ref{#1}}
% \newcommand{\myEqref}[1]{Equation~(\ref{#1})}
% \newcommand{\appref}[1]{\ref{#1}}
% \newcommand{\myappref}[1]{Appendix~\ref{#1}}
\newcommand{\myappref}[1]{\ref{#1}}
% \newcommand{\myAppref}[1]{Appendix~\ref{#1}}
\newcommand{\myAppref}[1]{\ref{#1}}
\newcommand{\mychapref}[1]{Chapter~\ref{#1}}
\newcommand{\myChapref}[1]{Chapter~\ref{#1}}

%% Comp. Mech format
% \newcommand{\figref}[1]{Fig.~\ref{#1}}
% \newcommand{\secref}[1]{Sect.~\ref{#1}}
% \newcommand{\chapref}[1]{Chap.~\ref{#1}}
% \newcommand{\tabref}[1]{Table~\ref{#1}}
% \renewcommand{\algref}[1]{Algorithm~\ref{#1}}

%% Standard format
% \newcommand{\figref}[1]{Figure~\ref{#1}}
% \newcommand{\Figref}[1]{Figure~\ref{#1}}
% \newcommand{\secref}[1]{section~\ref{#1}}
% \newcommand{\Secref}[1]{Section~\ref{#1}}
% \newcommand{\chapref}[1]{chapter~\ref{#1}}
% \newcommand{\Chapref}[1]{Chapter~\ref{#1}}
% \newcommand{\tabref}[1]{Table~\ref{#1}}
% \newcommand{\Tabref}[1]{Table~\ref{#1}}
% \providecommand{\algref}[1]{Algorithm~\ref{#1}}
% \renewcommand{\algref}[1]{Algorithm~\ref{#1}}
% \newcommand{\Algref}[1]{Algorithm~\ref{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Other commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Input from standard input path
\newcommand{\myinput}[1]{%
  \input{\CommonPath/#1}
}



%% footnotes
\newcounter{footnoteNumber} % initialization of counter with 0
\newcommand{\myfootnote}[1]
{% -> needed to avoid space between word and footnotemark
  \addtocounter{footnoteNumber}{1}%
  \footnotemark[\value{footnoteNumber}]%
  \footnotetext[\value{footnoteNumber}]{#1}%
}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "mainPhD"
%%% End: 


==> settings/myheadings.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % myheadings.tex
% %
% % 	requires:		\usepackage{scrpage2}
% % 				\usepackage{setspace}
% %

%%% Headings
%\pagestyle{headings}
\automark[chapter]{section}
\pagestyle{scrheadings}
% \rehead{\chaptermark}
\chead{}
\rohead[]{\pagemark}
%\rohead{\pagemark}
%\lohead{\rightmark}
\lohead{\rightmark}
\rehead{\leftmark}
% \lehead{}
\lehead{\pagemark}
\lefoot{}
\cefoot[]{}
\cofoot[]{}
% \rofoot[\pagemark]{\pagemark}
\rofoot[]{}
\setheadsepline{1pt}

%%% Vertical offset of chapters (standard is 1.8)
\renewcommand*{\chapterheadstartvskip}{\vspace{2.2\baselineskip}}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "mainPhD"
%%% End: 


==> settings/mytikzcommands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % mytikzcomments.tex
% %
% % 	requires:		\usepackage{tikz}
% % 				\usepackage{forloop}
% % 				\usepackage{arrayjobx}
% %

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% compatibility
\pgfplotsset{compat=1.10}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% externalize tikz-figures as graphics
\usetikzlibrary{external}
\tikzexternalize[optimize command away=\includepdf] 
%externalize ignores \includepdf objects
% \tikzexternalize[mode=list and make,prefix=tmp/]
% \tikzset{external/mode=list and make}
\tikzsetexternalprefix{tmp/}
% \tikzexternaldisable

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% TikZ additional packages
% \usetikzlibrary{positioning,calc,intersections,arrows,3d,fit}
% \usetikzlibrary{shapes,snakes,spy}
\usetikzlibrary{shapes,spy,fit}
% \usepgfplotslibrary{patchplots}
% \usetikzlibrary{matrix,chains,scopes,fit,decorations.pathmorphing} % for sim chain
% \usetikzlibrary{shapes.geometric,shapes.arrows,decorations.pathmorphing}
% \usetikzlibrary{matrix,chains,scopes,positioning,arrows,fit}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% PGF Plots additional packages
\usepgfplotslibrary{groupplots}
% \usepgfplotslibrary{fillbetween}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Font size in plots and graphics
\def\pgfplotfontsizetitle{\small}
\def\pgfplotfontsize{\footnotesize}
\def\tikzfontsize{\small}
\def\tikzfontsizesmall{\footnotesize}
\def\tikzfontsizetiny{\scriptsize}

\pgfplotsset{
  mystyle/.style ={%
    grid = major,
%     grid = none,
    every tick label/.append style={font=\pgfplotfontsize},
    every axis label/.append style={font=\pgfplotfontsize},
    legend style={font=\pgfplotfontsize},
    label style={font=\pgfplotfontsize},
    title style={font=\pgfplotfontsizetitle},
%       \pgfkeys{%
    /pgf/number format/set thousands separator = {}, % 1,000 -> 1000
%   }
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Custom drawing colors
% \definecolor{drawblue} {RGB}{87,117,225}
\colorlet{drawblue}      {blue!80!white}
% \definecolor{drawred}{RGB}{229,112,88}
\colorlet{drawred}       {red!80!white}
\colorlet{drawgray}      {gray}
% \definecolor{drawgreen}  {RGB}{0,.5,0}
\definecolor{drawgreen}  {RGB}{44,162,95}
% \definecolor{drawgreen}  {RGB}{49,163,84}
% \colorlet{drawgreen}  {olive}
\colorlet{drawpurple}    {purple}
\colorlet{draworange}    {orange}
\colorlet{drawlime}      {lime!80!black}
\colorlet{drawartichoke} {yellow!60!black}
\colorlet{TUGgray}{black!15}
\definecolor{TUGred}{RGB}{247,1,70}
\definecolor{IFBblue}{RGB}{51,112,169}
\definecolor{UTorange}{RGB}{191,87,0}
\definecolor{UTblue}{RGB}{0,95,134}
\definecolor{UTgreen}{RGB}{67,105,91}
\definecolor{UTgray}{RGB}{51,63,72}
\definecolor{UTyellow}{RGB}{242,169,0}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Custom basisfunction colors
\definecolor{basisColor1}{RGB}{59,76,192}
\definecolor{basisColor2}{RGB}{87,117,225}
\definecolor{basisColor3}{RGB}{119,154,247}
\definecolor{basisColor4}{RGB}{152,185,255}
\definecolor{basisColor5}{RGB}{184,208,249}
% \definecolor{basisColor6}{RGB}{213,219,230} % original settings
% \definecolor{basisColor7}{RGB}{236,211,197} % original settings
\definecolor{basisColor6}{RGB}{195,209,230}	% changed for printing
\definecolor{basisColor7}{RGB}{247,200,190}	% changed for printing
\definecolor{basisColor8}{RGB}{247,187,160}
\definecolor{basisColor9}{RGB}{244,154,123}
\definecolor{basisColor10}{RGB}{229,112,88}
\definecolor{basisColor11}{RGB}{203,62,56}
\definecolor{basisColor12}{RGB}{180,4,38}

\definecolor{basisColor8sw}{RGB} {189,189,189}
\definecolor{basisColor9sw}{RGB} {150,150,150}
\definecolor{basisColor10sw}{RGB}{115,115,115}
% \definecolor{basisColor11sw}{RGB}{82,82,82}
\definecolor{basisColor11sw}{RGB}{91,91,91}
\definecolor{basisColor12sw}{RGB}{37,37,37}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Custom plot colors and style

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Initial set 0 (standard TikZ)
\colorlet{myblue}    {blue}
\colorlet{myred}     {red}
% \definecolor{mygreen} {RGB}{44,162,95}
\colorlet{mygreen}   {drawgreen}
\colorlet{mypurple}  {purple}
\colorlet{myorange}  {orange}


%%% Set 1 - dark colors
%%% http://colorbrewer2.org, number of data classes=3, middle color
%% \definecolor{myblue}  {RGB}{43,140,190}
% \definecolor{myblue}  {RGB}{43,140,190}
% \definecolor{myred}   {RGB}{227,74,51}
% \definecolor{mygreen} {RGB}{44,162,95}
% \definecolor{mypurple}{RGB}{197,27,138}
% \definecolor{myorange}{RGB}{217,95,14}

%%% Set 2 - light colors
%%% http://colorbrewer2.org, number of data classes=3, middle color
% \definecolor{myblue}  {RGB}{166,189,219}
% \definecolor{myred}   {RGB}{253,187,132}
% \definecolor{mygreen} {RGB}{153,216,201}
% \definecolor{mypurple} {RGB}{250,159,181}
% \definecolor{myorange}{RGB}{254,196,79 }


%%% Cycle lists for plots


%%% Cyclelist 1 (custom)
% \pgfplotscreateplotcyclelist{mycyclelist}{
%   myblue,    every mark/.append style={solid, fill=.},mark=*          \\%
%   myred,     every mark/.append style={solid, fill=.},mark=square*     \\%
%   mygreen,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
%   mypurple,  every mark/.append style={solid, fill=.},mark=diamond*    \\%
%   % myorange,  every mark/.append style={solid, fill=.},mark=star    \\%
% }

% \pgfplotscreateplotcyclelist{mycyclelistcompare}{
%   myblue,    dashed            \\%
%   myred,     dotted            \\%
%   mygreen,   dashdotted        \\%
%   mypurple,  dashdotdotted     \\%
%   myblue,    only marks,   every mark/.append style={solid, fill=.},mark=*          \\%
%   myred,     only marks,   every mark/.append style={solid, fill=.},mark=square*     \\%
%   mygreen,   only marks,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
%   mypurple,  only marks,   every mark/.append style={solid, fill=.},mark=diamond*    \\%
% }

%%% Cyclelist 2 (TikZ exotic)
% \pgfplotscreateplotcyclelist{mycyclelist}{
%   teal,    every mark/.append style={solid, fill=.},mark=*           \\%
%   orange,  every mark/.append style={solid, fill=.},mark=square*     \\%
%   cyan,    every mark/.append style={solid, fill=.},mark=triangle*   \\%
%   red,     every mark/.append style={solid, fill=.},mark=diamond*    \\%
%   % lime,  every mark/.append style={solid, fill=.},mark=diamond*    \\%
% }

% %%% Cyclelist 3 (TikZ standard)
% \pgfplotscreateplotcyclelist{mycyclelist}{
% %     \pgfplotscreateplotcyclelist{color}{%
% blue,every mark/.append style={fill=blue!80!black},mark=*\\%
% red,every mark/.append style={fill=red!80!black},mark=square*\\%
% brown!60!black,every mark/.append style={fill=brown!80!black},mark=otimes*\\%
% black,mark=star\\%
% blue,every mark/.append style={fill=blue!80!black},mark=diamond*\\%
% red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=*\\%
% brown!60!black,densely dashed,every mark/.append style={
% solid,fill=brown!80!black},mark=square*\\%
% black,densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
% blue,densely dashed,mark=star,every mark/.append style=solid\\%
% red,densely dashed,every mark/.append style={solid,fill=red!80!black},mark=diamond*\\%
% % }
% %   blue,    every mark/.append style={solid, fill=.},mark=*           \\%
% %   red,     every mark/.append style={solid, fill=.},mark=square*     \\%
% %   brown,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
% %   black,   every mark/.append style={solid, fill=.},mark=diamond*    \\%
% }

%%% Cyclelist 4 (red styles)

% % \ifthenelse{\boolean{isbook}}{ 
% % % \definecolor{basisColor11new}{RGB}{203,80,56}
% % 
% % %% gray styles
% % \pgfplotscreateplotcyclelist{mycyclelist}{
% %   basisColor12sw,semithick, every mark/.append style={solid, fill=.},mark=*           \\%
% %   basisColor11sw,semithick, every mark/.append style={solid, fill=.},mark=square*     \\%
% %   basisColor10sw,semithick, every mark/.append style={solid, fill=.},mark=triangle*   \\%
% %   basisColor9sw , semithick,every mark/.append style={solid, fill=.},mark=diamond*    \\%
% %   basisColor8sw , semithick,every mark/.append style={solid, fill=.},mark=otimes    \\%
% % }
% % %% based on "linestyles*", pgfplots documentation S.199
% % % \pgfplotscreateplotcyclelist{mycyclelist}{
% % % semithick,darkgray,solid,        mark=*             \\%
% % % semithick,darkgray,dashed,       mark=square*       \\%
% % % semithick,darkgray,dotted,       mark=triangle*     \\%
% % % semithick,darkgray,dashdotted,   mark=diamond*      \\%
% % % semithick,darkgray,dashdotdotted,mark=otimes        \\%
% % % }
% % % %% copy of "black white", pgfplots documentation S.198 
% % % \pgfplotscreateplotcyclelist{mycyclelist}{
% % % every mark/.append style={fill=gray},mark=*\\%
% % % every mark/.append style={fill=gray},mark=square*\\%
% % % % every mark/.append style={fill=gray},mark=otimes*\\%
% % % mark=star\\%
% % % every mark/.append style={fill=gray},mark=diamond*\\%
% % % densely dashed,every mark/.append style={solid,fill=gray},mark=*\\%
% % % densely dashed,every mark/.append style={solid,fill=gray},mark=square*\\%
% % % % densely dashed,every mark/.append style={solid,fill=gray},mark=otimes*\\%
% % % densely dashed,every mark/.append style={solid},mark=star\\%
% % % densely dashed,every mark/.append style={solid,fill=gray},mark=diamond*\\%
% % % }
% % % %% end copy
% % }{

%% red styles
% \pgfplotscreateplotcyclelist{mycyclelist}{
%   basisColor12,semithick,   every mark/.append style={solid, fill=.},mark=*           \\%
%   basisColor11,semithick,   every mark/.append style={solid, fill=.},mark=square*     \\%
%   basisColor10,semithick,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
%   basisColor9, semithick,   every mark/.append style={solid, fill=.},mark=+    \\%
%   basisColor8, semithick,   every mark/.append style={solid, fill=.},mark=otimes    \\%
% }
% % %
% % }

% %%% Cyclelist 5 comparison for trimmed cube example
\pgfplotscreateplotcyclelist{mycyclelist}{
blue,every mark/.append style={fill=blue!80!black},mark=*\\%
red,every mark/.append style={fill=red!80!black},mark=square*\\%
brown!60!black,dashed,every mark/.append style={fill=brown!80!black},mark=otimes*\\%
black,dashed,mark=star\\%
}


% \definecolor{cyclelistRed}{RGB}{228,26,28}
% \definecolor{cyclelistBlue}{RGB}{55,126,184}
% \definecolor{cyclelistGreen}{RGB}{77,175,74}
% \definecolor{cyclelistViolette}{RGB}{152,78,163}
% \pgfplotscreateplotcyclelist{mycyclelistcompare}{
%   cyclelistRed,     semithick, solid               	\\%
%   cyclelistBlue,    semithick, loosely dashdotted        \\%
%   cyclelistGreen,   semithick, dashed      		\\%
%   cyclelistViolette,semithick, loosely dashdotdotted     \\%
%   cyclelistRed,     only marks,   every mark/.append style={solid, fill=.},mark=*          \\%
%   cyclelistBlue,    only marks,   every mark/.append style={solid, fill=.},mark=square*     \\%
%   cyclelistGreen,   only marks,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
%   cyclelistViolette,only marks,   every mark/.append style={solid, fill=.},mark=diamond*    \\%
% }

%% red and blue styles
% \pgfplotscreateplotcyclelist{mycyclelistcompare}{
%   basisColor1,     semithick, solid               	\\%
%   basisColor10,    semithick, loosely dashdotted        \\%
%   basisColor3,   semithick, dashed      		\\%
%   basisColor12,semithick, loosely dashdotdotted     \\%
%   basisColor1,     only marks,   every mark/.append style={solid, fill=.},mark=*          \\%
%   basisColor10,    only marks,   every mark/.append style={solid, fill=.},mark=square*     \\%
%   basisColor3,   only marks,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
%   basisColor12,only marks,   every mark/.append style={solid, fill=.},mark=diamond*    \\%
% }

% % \ifthenelse{\boolean{isbook}}{ 
% % %% gray styles
% % \pgfplotscreateplotcyclelist{mycyclelistcompare}{
% %   basisColor12sw, semithick, loosely dashdotdotted     \\%
% %   basisColor11sw, semithick, loosely dashed      		\\%
% %   basisColor10sw, semithick, dashed \\%loosely dashdotted        \\%
% %   basisColor9sw,  semithick, solid               	\\%
% %   basisColor12sw, only marks,   every mark/.append style={solid, fill=.},mark=otimes    \\%
% %   basisColor11sw, only marks,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
% %   basisColor10sw, only marks,   every mark/.append style={solid, fill=.},mark=square*     \\%
% %   basisColor9sw,  only marks,   every mark/.append style={solid, fill=.},mark=*          \\%
% % }
% % %
% % 
% % }{
%% red styles
\pgfplotscreateplotcyclelist{mycyclelistcompare}{
  basisColor12, semithick, loosely dashdotdotted     \\%
  basisColor11, semithick, loosely dashed      		\\%
  basisColor10, semithick, dashed \\%loosely dashdotted        \\%
  basisColor9,  semithick, solid               	\\%
  basisColor12, only marks,   every mark/.append style={solid, fill=.},mark=otimes    \\%
  basisColor11, only marks,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
  basisColor10, only marks,   every mark/.append style={solid, fill=.},mark=square*     \\%
  basisColor9,  only marks,   every mark/.append style={solid, fill=.},mark=*          \\%
}
% % %
% % }

% % \ifthenelse{\boolean{isbook}}{ 
% % %% gray styles
% % \tikzset{mycyclelistcompareReferenceA/.style={basisColor12sw,solid}}
% % \tikzset{mycyclelistcompareTestA/.style={basisColor12sw,only marks,mark=otimes}}
% % }{
%% red styles
\tikzset{mycyclelistcompareReferenceA/.style={basisColor12,solid}}
\tikzset{mycyclelistcompareTestA/.style={basisColor12,only marks,mark=otimes}}
% % }
% \pgfplotscreateplotcyclelist{mycyclelistcompareToReference}{
%   basisColor9, very thick, loosely dashed    \\%
%   basisColor12, solid\\%
% %   basisColor11, semithick, loosely dashed      		\\%
% %   basisColor10, semithick, dashed \\%loosely dashdotted        \\%
% %   basisColor9,  semithick, solid               	\\%
% %   basisColor12, only marks,mark=otimes    \\%
% %   basisColor11, only marks,   every mark/.append style={solid, fill=.},mark=triangle*   \\%
% %   basisColor10, only marks,   every mark/.append style={solid, fill=.},mark=square*     \\%
% %   basisColor9,  only marks,   every mark/.append style={solid, fill=.},mark=*          \\%
% }



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Additional styles

%% line styles
\tikzset{helpline/.style={thin,dashed}}
\tikzset{labelline/.style={thin}}
\tikzset{referencePath/.style={dotted,very thick}}
\tikzset{helparrow/.style={thin,arrows={-latex}}}
% \tikzset{pointer/.style={arrows={latex-latex}}}
\tikzset{pointer/.style={arrows={-latex}}}
\tikzset{axis/.style={thin,arrows={->}}}
\tikzset{force/.style={thick,arrows={->}}}
\tikzset{forceInverse/.style={thick,arrows={<-}}}
\tikzset{Gamma/.style={ultra thick}}
\tikzset{controlPoly/.style={draw=black}}
\tikzset{GammaFill/.style={fill=lightgray,fill opacity=0.3}}
\tikzset{colorDiri/.style={drawgreen}}
\tikzset{GammaFillDiri/.style={fill=drawgreen,fill opacity=0.5}}
\tikzset{initialgrid/.style={thin,gray}}
\tikzset{intersectioncurve/.style={dashed,thick}}
\tikzset{trimmingcurve/.style={thick}}
\tikzset{boundingbox/.style={dashed,}}
\tikzset{approx/.style={thick,line join=round,dashed}}
\tikzset{integrationRegionEdge/.style={dashed}}

%% point styles
\tikzstyle{anode}= [circle, inner sep=1.3pt, draw, fill=black]
\tikzstyle{gausspoint}=[shape=circle,draw=black,fill=black,inner sep=0.8pt]
\tikzstyle{controlPoint}=[shape=circle,draw=black,fill=white,thin,inner sep=0pt,minimum size=1.5mm]
\tikzstyle{abscissaPoint}=[shape=circle,draw=black,fill=white,thin,inner sep=0pt,minimum size=1.5mm]
\tikzstyle{anchorPoint}=[shape=circle,draw=black,fill=black,thin,inner sep=0pt,minimum size=1.5mm]
% \tikzstyle{anchorPointDeg}=[shape=circle,draw=black,fill=white,thin,inner sep=0pt,minimum size=1.5mm]
\tikzstyle{anchorPointDeg}=[shape=cross out,thick,draw=black,inner sep=0pt,minimum size=1.5mm]
\tikzstyle{trimmingIntersectionPoint}=[shape=cross out,thick,draw=black,inner sep=0pt,minimum size=1.5mm]
\tikzstyle{approxnode}= [circle, inner sep=1.5pt, draw, fill=black]
% \tikzstyle{characterNode}= [rectangle, inner sep=1.8pt, draw,thick,fill=white]
\tikzstyle{characterNode}= [shape=cross out,rotate=45, inner sep=1.8pt, draw,very thick,fill=white]

\tikzstyle{aPointPatchA}= [circle, inner sep=1.3pt, draw, fill=black]
\tikzstyle{aPointPatchB}= [circle, inner sep=1.3pt, draw, fill=white]
\tikzstyle{aPointModelSpace}=[shape=cross out,thick,draw=black,inner sep=0pt,minimum size=1.5mm]


% \tikzstyle{anchorPoint}=[shape=circle,draw=black,fill=black,inner sep=0pt,minimum size=1.5mm]%, maximum size=1.5mm]
% \tikzstyle{anchorPointDisp}=[shape=circle,draw=black,fill=drawgreen,inner sep=0pt,minimum size=1.5mm]%, maximum size=1.5mm]
% \tikzstyle{collocPoint}=[shape=rectangle,draw=black,fill=black,thick,inner sep=0pt,minimum size=1.2mm] %, maximum size=1.2mm] 
% \tikzset{Diri/.style={drawgreen}}
% \tikzset{Neum/.style={drawpurple}}
% \tikzset{collocNeum/.style={collocPoint, fill=drawgreen}}
% \tikzset{collocDiri/.style={collocPoint, fill=drawpurple}}
% 
% \tikzset{GammaDiri/.style={Gamma, Diri}}
% \tikzset{GammaNeum/.style={Gamma, Neum}}
% 
% \tikzset{anchorNeum/.style={anchorPoint, fill=drawpurple}}
% \tikzset{anchorDiri/.style={anchorPoint, fill=drawgreen}}
% 
% \tikzset{helpline/.style={thin,dashed}}
% \tikzset{helpline/.style={thin}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% help makro for convergence plots

\def\trianglecolor{black}
\newcommand{\upperSlopeTriangle}[4] 	% input: #1 slope #2 vertical shift  #3 min x-value #4 max x-value
								% example call: \upperSlopeTriangle{2}{100}{1000}{5000}
{
	\addplot[forget plot, domain=#3:#4,color=\trianglecolor,samples=2]{  #2 / (x^#1) } node (A1) [pos=1] {}; 
	\addplot[forget plot, domain=#3:#4,color=\trianglecolor,samples=2]{   #2  / (#3^#1)} node (A2) [pos=1] {} node [anchor=south,pos=0.5,black] {\tikzfontsizetiny $1$};
	\draw[color=\trianglecolor] (A1.center) -- (A2.center) node [anchor=west,pos=0.5,black] {\tikzfontsizetiny #1};
}

\newcommand{\lowerSlopeTriangle}[4] 	% input: #1 slope #2 vertical shift  #3 min x-value #4 max x-value
								% example call: \lowerSlopeTriangle{2}{100}{1000}{5000}
{
% 	\def\trianglecolor{black}
	\addplot[forget plot, domain=#3:#4,color=\trianglecolor,samples=2]{  #2 / (x^#1) } node (A1) [pos=0] {}; 
	\addplot[forget plot, domain=#3:#4,color=\trianglecolor,samples=2]{   #2  / (#4^#1)} node (A2) [pos=0] {} node [anchor=north,pos=0.5,black] {\tikzfontsizetiny $1$};
	\draw[color=\trianglecolor] (A1.center) -- (A2.center) node [anchor=east,pos=0.5,black] {\tikzfontsizetiny #1};
}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% B-spline functions

\newcounter{itR}
\newcommand{\bsplinevalue}[5] % input: #1 knot vector #2 order,  #3 intrinsic coordinate #4 span index #5 output name
						% remark: #1 has to be parsed explicitly ( \def\vKnots{...} \bsplinevalue{\vKnots}{×}{×}{×}{×} fails!  )
{                    				
	\newarray\vKnots
	\newarray\vN
	\newarray\vNumeratorL
	\newarray\vNumeratorR
	\newarray\vSave

	\readarray{vKnots}{#1}
	\readarray{vN}{1}
	\readarray{vSave}{0}
	\readarray{vNumeratorL}{0}
	\readarray{vNumeratorR}{0}

	\foreach \j in {1,...,#2}
	{        
		\pgfmathparse{ int(#4+\j+1) } \checkvKnots(\pgfmathresult)
		\pgfmathsetmacro{\numR}{\cachedata-#3}
		
		\pgfmathparse{ int(#4-\j+2) } \checkvKnots(\pgfmathresult)
		\pgfmathsetmacro{\numL}{#3-\cachedata} 					

		\expandarrayelementtrue
		\pgfmathparse{ int(\j+1) }
		\vNumeratorL(\pgfmathresult)={\numL}
		\vNumeratorR(\pgfmathresult)={\numR}
		
		\forloop[1]{itR}{0}{\value{itR} < \j }
		{
			\pgfmathparse{ int(\theitR+1) } \let\tS\pgfmathresult  	
			\checkvSave(\tS)							
			\pgfmathsetmacro{\save}{\cachedata}  
		
			\pgfmathparse{int(\j-\theitR+1)} \checkvNumeratorL(\pgfmathresult)
			\pgfmathsetmacro{\tmpL}{\cachedata} 	
		    
			\pgfmathparse{ int(\theitR+2) } \checkvNumeratorR(\pgfmathresult)
			\pgfmathsetmacro{\tmpR}{\cachedata} 	       
	
			\pgfmathparse{ int(\theitR+1) } \checkvN(\pgfmathresult)
			\pgfmathparse{ \cachedata / (\tmpL+\tmpR) } \let\tmp\pgfmathresult
			
			\pgfmathparse{ \save + \tmpR * \tmp } 
			\vN(\tS)={\pgfmathresult}

			\pgfmathparse{ \tmpL * \tmp } \let\tmpsave\pgfmathresult
			\pgfmathparse{ int(\theitR+2) } \let\tS\pgfmathresult      
			\vSave(\tS)={\tmpsave}
		}
		
		\pgfmathparse{ int(\j+1) } \checkvSave(\pgfmathresult )
		\vN(\tS)={\cachedata}
	}

	% write to return argument #5
	\pgfmathparse{int( #2+1) } \let\lastIndex\pgfmathresult
	\checkvN(1) \pgfmathsetmacro{\first}{\cachedata}  
	\foreach \i [remember=\a as \lasta (initially \first)] in {2,...,\lastIndex}
	{
		\checkvN(\i) \def\a{\lasta,\cachedata} 
		% store \a of last loop
		\ifthenelse{\i=\lastIndex}{ \xdef#5{\a} }{}
	}
    
	% clean up
	\foreach \i in {1,...,\lastIndex}
	{
	    \clrarray{vNumeratorR}(\i)
	    \clrarray{vNumeratorL}(\i)
	    \clrarray{vN}(\i)
	    \clrarray{vSave}(\i)
	}
	\delarray\vN
	\delarray\vNumeratorL
	\delarray\vNumeratorR
	\delarray\vSave
}

\newcounter{countvalues}
\newcounter{getBasis}
\newcommand{\bsplinebasis}[4] % input: #1 knot vector, #2 order,  #3 id of basis function, #4 output
{						% example: \bsplinebasis{0&0&0&1&2&2&2}{2}{0}{\output}
						% remark: #1 has to be parsed explicitly ( \def\vKnots{...} \bsplinebasis{\vKnots}{×}{×}{×} fails!  )
						%		countvalues returns the number of non-zero basis functions
						%		\output ''intrinsic Coord, basis function value'': ''u0,N_#3(u0)'',''u1,N_#3(u1)'',...,''un,N_#3(un)''
    \newarray\vKnots 	% remark index start from 1
    \readarray{vKnots}{#1}

    \pgfmathparse{#3}  \let\i\pgfmathresult
    \pgfmathparse{#2}  \let\p\pgfmathresult

    % loop over support of N_i
    \setcounter{countvalues}{0}
    \setcounter{getBasis}{\p} %\addtocounter{getBasis}{1}
    \pgfmathparse{int(\i+\p)}
    \foreach \knotspan in {\i,...,\pgfmathresult}
    {
        % check span size
	\pgfmathparse{ int(\knotspan+1+1) } \checkvKnots(\pgfmathresult)
	\pgfmathsetmacro{\tmpR}{\cachedata} 						%R: \tmpR
	
	\pgfmathparse{ int(\knotspan+1) } \checkvKnots(\pgfmathresult) 
	\pgfmathsetmacro{\tmpL}{\cachedata} 						%L: \tmpL

	\pgfmathparse{ \tmpR - \tmpL } \let\spansize\pgfmathresult  			%S: \spansize 
   
        \pgfmathparse{ \spansize > 0.0 } \let\bNonZero\pgfmathresult
        \ifthenelse{ \bNonZero = 1 }
        {
            % evaluate points \u with in the span
            \foreach \percentU in {0,10,...,100}
            {
		\pgfmathparse{\tmpL+\spansize*\percentU/100} \let\u\pgfmathresult

		% get all non vanishing basis functions
		\bsplinevalue{#1}{\p}{\u}{\knotspan}{\Basis} 
		\def\basisfuncarray{{\Basis}} 				% remark index start from 0
		
		\pgfmathparse{\basisfuncarray[\thegetBasis]} %\pgfmathresult
		
		\ifthenelse{\thecountvalues=0}
		{ 
			\xdef\nodeB{"\u,\pgfmathresult"}
		}{
			\xdef\nodeB{\nodeB,"\u,\pgfmathresult"}  
		}
		\addtocounter{countvalues}{1}
            }
        }{}
        \addtocounter{getBasis}{-1}
    }
    
	\xdef#4{\nodeB}

	\delarray\vKnots
}


\newcommand{\bsplinebasisspan}[6] % input: 	#1 knot vector, #2 order,  #3 segment id of basis function within (#4), 
{							% 		#4 id of knot span,  #5 id of plotted span, #6 output
							% example: \bsplinebasis{0&0&0&1&2&2&2}{2}{0}{\output}
							% remark: #1 has to be parsed explicitly ( \def\vKnots{...} \bsplinebasis{\vKnots}{×}{×}{×} fails!  )
							%		#3 is not  the basis function id 
							%		   - for each span the numbering start at 0 - index first non-zero basis function of #4
							%		countvaluesspan returns the number of non-zero basis functions
							%		\output ''intrinsic Coord, basis function value'': ''u0,N_#3(u0)'',''u1,N_#3(u1)'',...,''un,N_#3(un)''
    \newarray\vKnots 	% remark index start from 1
    \readarray{vKnots}{#1}

    \pgfmathparse{#5}  \let\plotknotspan\pgfmathresult
    \pgfmathparse{#4}  \let\splineknotspan\pgfmathresult
    \pgfmathparse{#3}  \let\i\pgfmathresult
    \pgfmathparse{#2}  \let\p\pgfmathresult

    % only one iteration over support '\plotknotspan' 
    % evaluation the polynome defined over '\splineknotspan'
    \setcounter{countvalues}{0}
    \setcounter{getBasis}{\i} 
    \foreach \knotspan in {\plotknotspan}
    {
        % check span size
	\pgfmathparse{ int(\knotspan+1+1) } \checkvKnots(\pgfmathresult)
	\pgfmathsetmacro{\tmpR}{\cachedata} 						%R: \tmpR
	
	\pgfmathparse{ int(\knotspan+1) } \checkvKnots(\pgfmathresult) 
	\pgfmathsetmacro{\tmpL}{\cachedata} 						%L: \tmpL

	\pgfmathparse{ \tmpR - \tmpL } \let\spansize\pgfmathresult  			%S: \spansize 
   
        \pgfmathparse{ \spansize > 0.0 } \let\bNonZero\pgfmathresult
        \ifthenelse{ \bNonZero = 1 }
        {
            % evaluate points \u with in the span
            \foreach \percentU in {0,10,...,100}
            {
		\pgfmathparse{\tmpL+\spansize*\percentU/100} \let\u\pgfmathresult

		% get all non vanishing basis functions
		\bsplinevalue{#1}{\p}{\u}{\splineknotspan}{\Basis} 
		\def\basisfuncarray{{\Basis}} 				% remark index start from 0
		
		\pgfmathparse{\basisfuncarray[\thegetBasis]} %\pgfmathresult
		
		\ifthenelse{\thecountvalues=0}
		{ 
			\xdef\nodeB{"\u,\pgfmathresult"}
		}{
			\xdef\nodeB{\nodeB,"\u,\pgfmathresult"}  
		}
		\addtocounter{countvalues}{1}
            }
        }{}
        \addtocounter{getBasis}{-1}
    }
    
	\xdef#6{\nodeB}

	\delarray\vKnots
}





\newcommand{\plotbsplinebasis}[4] 	% input: #1 knot vector, #2 order,  #3 id of basis function, #4 plot settings
{							% example: \plotbsplinebasis{0&0&0&1&2&2&2}{2}{0}{green,smooth}
							% remark: #1 has to be parsed explicitly ( \def\vKnots{...} \plotbsplinebasis{\vKnots}{×}{×}{×} fails!  )
	% calculate B-spline values
	\bsplinebasis{#1}{#2}{#3}{\nodeOut}
	\def\nodearray{{\nodeOut}}

	% store B-spline values into coordinates and save their name
	\xdef\name{ }
	\addtocounter{countvalues}{-1}
	\foreach \i in {0,...,\thecountvalues}
	{
		\pgfmathparse{\nodearray[\i]}
		\coordinate (point\i) at (\pgfmathresult);	  
		\xdef\name{ \name (point\i)  }
	}
	
	% plot basis
	\draw[#4] plot coordinates{ \name };
	
	% reset coordinates
	\xdef\name{ }
}


\newcommand{\plotbsplinesegment}[6] 	% input: 	#1 knot vector, #2 order,  #3 segment id of basis function within (#4),  
{								%		#4 id of knot span, #5 id of plotted span, #6 plot settings
								% example: 
								%	->normal B-spline plot
								% 	\plotbsplinebasis{0&0&0&1&2&3&3&3}{2}{1}{basisColor3,dotted,thick}
								%	\plotbsplinebasis{0&0&0&1&2&3&3&3}{2}{2}{basisColor5,dotted,thick}
								%	\plotbsplinebasis{0&0&0&1&2&3&3&3}{2}{3}{basisColor7,dotted,thick}
								%	
								%	-> plot the B-spline segments 0,1,2 of span 3 in span 2
								%
								%	\plotbsplinesegment{0&0&0&1&2&3&3&3}{2}{0}{3}{2}{red,smooth}
								%	\plotbsplinesegment{0&0&0&1&2&3&3&3}{2}{1}{3}{2}{red,smooth}
								%	\plotbsplinesegment{0&0&0&1&2&3&3&3}{2}{2}{3}{2}{blue,smooth}
								%
								% remark: #1 has to be parsed explicitly ( \def\vKnots{...} \plotbsplinebasis{\vKnots}{×}{×}{×} fails!  
								
	% calculate B-spline values
	\bsplinebasisspan{#1}{#2}{#3}{#4}{#5}{\nodeOut}
	\def\nodearray{{\nodeOut}}

	% store B-spline values into coordinates and save their name
	\xdef\name{ }
	\addtocounter{countvalues}{-1}
	\foreach \i in {0,...,\thecountvalues}
	{
		\pgfmathparse{\nodearray[\i]}
		\coordinate (point\i) at (\pgfmathresult);	  
		\xdef\name{ \name (point\i)  }
	}
	
	% plot basis
	\draw[#6] plot coordinates{ \name };
	
	% reset coordinates
	\xdef\name{ }
}


\newcommand{\plotbsplineaccumulated}[5] 	% input: 	#1 knot vector, #2 order,  #3 subdivision coefficient,  
{						%		#4 id of knot span,  #5 plot settings
						% example: 
                                                %       ->plot non-zero basis function segment within #4
						%	\plotbsplineaccumulated{0&0&0&1&2&3&3&3}{2}{1&0&0}{3}{red,smooth}
						% 	\plotbsplineaccumulated{0&0&0&1&2&3&3&3}{2}{0&1&0}{3}{green,smooth}
						%	\plotbsplineaccumulated{0&0&0&1&2&3&3&3}{2}{0&0&1}{3}{blue,smooth}
                                                %       
                                                %       ->plot weighted combination of basis function segments within #4
						%	\plotbsplineaccumulated{0&0&0&1&2&3&3&3}{2}{0&1&1}{3}{blue,smooth}
						%	
						% remark: #1 has to be parsed explicitly ( \def\vKnots{...} \plotbsplinebasis{\vKnots}{×}{×}{×} fails!  

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%                                                            
    %% calculate B-spline values and compute their weighted sum using vSubCoef
    \newarray\vKnots 	% remark index start from 1
    \readarray{vKnots}{#1}
    \newarray\vSubCoef 	% remark index start from 1
    \readarray{vSubCoef}{#3}
    
    \pgfmathparse{#4}  \let\plotknotspan\pgfmathresult
    \pgfmathparse{#4}  \let\splineknotspan\pgfmathresult
    \pgfmathparse{#2}  \let\p\pgfmathresult
    
    % only one iteration over support '\plotknotspan' 
    % evaluation the polynome defined over '\splineknotspan'
    \setcounter{countvalues}{0}
    \pgfmathparse{int( \p+1) } \let\lastIndex\pgfmathresult
    \foreach \knotspan in {\plotknotspan}
    {
        % check span size
        \pgfmathparse{ int(\knotspan+1+1) } \checkvKnots(\pgfmathresult)
        \pgfmathsetmacro{\tmpR}{\cachedata} 						%R: \tmpR
        
        \pgfmathparse{ int(\knotspan+1) } \checkvKnots(\pgfmathresult) 
        \pgfmathsetmacro{\tmpL}{\cachedata} 						%L: \tmpL
        
        \pgfmathparse{ \tmpR - \tmpL } \let\spansize\pgfmathresult  			%S: \spansize 
        
        \pgfmathparse{ \spansize > 0.0 } \let\bNonZero\pgfmathresult
        \ifthenelse{ \bNonZero = 1 }
        {
            % evaluate points \u with in the span
            \foreach \percentU in {0,10,...,100}
            {
                \pgfmathparse{\tmpL+\spansize*\percentU/100} \let\u\pgfmathresult
                
                % get all non vanishing basis functions
                \bsplinevalue{#1}{\p}{\u}{\splineknotspan}{\Basis} 
                \def\basisfuncarray{{\Basis}} 				% remark index start from 0
                
                \setcounter{getBasis}{0} 
                \pgfmathparse{\basisfuncarray[\thegetBasis]} %\pgfmathresult
                \let\basisValue\pgfmathresult
                
                \checkvSubCoef(1) \pgfmathsetmacro{\coef}{\cachedata}  
                \pgfmathparse{ \basisValue * \coef } \let\first\pgfmathresult
                
                \xdef\lastx{\first}
                \foreach \i in {2,...,\lastIndex}
                { 
                    \addtocounter{getBasis}{1}       
                    \pgfmathparse{\basisfuncarray[\thegetBasis]}
                    \let\basisValue\pgfmathresult
                    
                    \checkvSubCoef(\i) \pgfmathsetmacro{\coef}{\cachedata}  
                    \pgfmathparse{ \lastx + \basisValue * \coef } \let\sum\pgfmathresult
                    
                    \xdef\lastx{\sum}
                    
                    % store \a of last loop
                    \ifthenelse{\i=\lastIndex}
                    {
                        \ifthenelse{\thecountvalues=0}
                        { 
                            \xdef\nodeBB{"\u,\sum"}
                        }{
                            \xdef\nodeBB{\nodeBB,"\u,\sum"}  
                        }
                        \addtocounter{countvalues}{1}
                    }{}
                    
                }
            }
        }{}
    }
    
    \delarray\vKnots
    \delarray\vSubCoef
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%
    %% plot accumulated values
    \def\nodearray{{\nodeBB}}
    
    % store B-spline values into coordinates and save their name
    \xdef\name{ }
    \addtocounter{countvalues}{-1}
    \foreach \i in {0,...,\thecountvalues}
    {
        \pgfmathparse{\nodearray[\i]}
        \coordinate (point\i) at (\pgfmathresult);                
        \xdef\name{ \name (point\i)  }
    }
    
    % plot basis
    \draw[#5] plot coordinates{ \name };
    
    % reset coordinates
    \xdef\name{ }
}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "mainPhD"
%%% End: 


==> settings/settings_font.tex <==
\usepackage[utf8]{inputenc} % for UTF-8 encoding
\usepackage[german,english]{babel}  
\usepackage[T1]{fontenc} % größerer Zeichenvorat z.B. für Umlaute 
\usepackage{lmodern} % latin modern fonts - added to resolve visualization issues with fontenc

% \usepackage{times} % times font
% \usepackage{mathptmx}  % times roman, including math (where possible)

%%% Hyphenations 
%\hyphenation{fast-bem}
% 


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> settings/settings_math.tex <==
\usepackage[intlimits]{amsmath}
\usepackage{amssymb} 
\usepackage{amsthm}
% \usepackage{amsbsy}
\usepackage{amsfonts,mathrsfs}
\usepackage{bm}
% \usepackage{mathdots} % for \iddots
\usepackage{mathtools} % for \coloneqq and \shortintertext


%%%% Tensors, Matrices and Vectors
% \usepackage[arrow]{hhtensor}
% \usepackage[uline]{hhtensor}
% \usepackage[bold]{hhtensor}
%%%%%%%%%%%

\usepackage{siunitx} %% units

% \usepackage{amsfonts,mathrsfs,bbm}
% \usepackage{amsfonts,mathrsfs}

%\usepackage{mathrsfs} 
%\usepackage{nicefrac}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "fastigabem"
%%% eval:
%%% End: 


==> settings/settings_tools.tex <==
%%% TikZ Stuff
\usepackage{tikz}
\usepackage{tikz-3dplot}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage{tikzscale}
\usepackage{standalone} % for standalone compilation of tikz graphics

%%% TikZ B-spline plots
\usepackage{forloop}
\usepackage{arrayjobx}

%%% algorithms
\usepackage[noend]{algorithmic}
\usepackage{algorithm}

\usepackage{booktabs} % for tables: toprule, midrule, bottomrule
\usepackage{hyperref} % for links -> this will be loaded by pdfcomment package
% \usepackage{calc}
\usepackage{xspace} % horizontal space after makro words

%% packages for authors' notes
\usepackage{xcolor,pdfcomment,soul} % add pdf comments
\usepackage[textsize=footnotesize]{todonotes}
% \usepackage[textsize=footnotesize,textwidth=1.2cm]{todonotes}
% \setlength{\marginparwidth}{1.2cm}

%%% subcaptions for figures
\usepackage{subcaption} 			%% 1a
\usepackage[labelformat=simple]{subcaption}   	%% 1(a)
\renewcommand\thesubfigure{(\alph{subfigure})}	%% 1(a)

\usepackage{enumerate} %% symbols for enumeration


% \usepackage{listings} %% enviroment for code formating 

==> tikz/new_commands.tex <==
%% SHORTCUTS
\newcommand{\Bezier}{B\'ezier~}

%% MATH NOTATION MACROS
%\newcommand{\mat}[1]{\mathbf{#1}} 
%\newcommand{\vect}[1]{\boldsymbol{\mathbf{#1}}}
\newcommand{\mat}[1]{\mathsf{#1}} 
\newcommand{\vect}[1]{#1}
\newcommand{\List}[1]{\left(\right. #1 \left.\right) }
\newcommand{\eigfun}{\phi}
\newcommand{\deigfun}{\phi_h}
\newcommand{\eigval}{\lambda}
\newcommand{\eigvec}{\mat{v}_h}
\newcommand{\eigveci}[1]{v_{h,{\midx{#1}}}}
\newcommand{\x}{\vect{x}}
\newcommand{\xp}{\vect{x}^\prime}
\newcommand{\px}{\hat{\x}}
\newcommand{\pxp}{\hat{\x}^\prime}
\newcommand{\pxk}[1]{\hat{\x}_{#1}}
\newcommand{\pxpk}{\hat{\x}^\prime}
\newcommand{\transposed}[1]{{#1}^\top}
\newcommand{\invtransposed}[1]{{#1}^{-\top}}
\newcommand{\dint}[1]{\,\mathrm{d}{#1}}
\newcommand{\ddint}[1]{\mathrm{d}{#1}}
\newcommand{\midx}[1]{\mathsf{#1}}

\newcommand{\bsspace}[1]{\mathcal{B}_{#1}}
\newcommand{\tbsspace}[1]{\tilde{\mathcal{B}}_{#1}}
\newcommand{\ubspline}[2]{B_{#1,#2}}
\newcommand{\bspline}[1]{B_{\midx{#1}}}
\newcommand{\geomap}[1]{F(#1)}
\newcommand{\geomapNOARG}[1]{F}
\newcommand{\bsplineNOARG}[1]{B_{\midx{#1}}}
\newcommand{\invgeomap}[1]{F^{-1}(#1)}
\newcommand{\detgeomap}[1]{\mathrm{det}\,\mathrm D\geomap{#1}}
\newcommand{\detgeomapNOARG}{\mathrm{det}\,\mathrm D\geomapNOARG}
\newcommand{\detinvgeomap}[1]{\mathrm{det}\,\mathrm D\invgeomap{#1}}

\newcommand{\approxdom}{\tilde{\mathcal D}}
\newcommand{\tbspline}[2]{\tilde{B}_{\midx{#1}}(#2)}
\newcommand{\tubspline}[3]{\tilde B_{#1,#2}(#3)}
\newcommand{\interpmat}[2]{B_{#1 #2}}
\newcommand{\tinterpmat}[2]{\tilde{B}_{#1 #2}}
\newcommand{\invinterpmat}[2]{B^{-1}_{#1 #2}}

\newcommand{\matinterpmat}{\mat B}
\newcommand{\tmatinterpmat}{\mat{\tilde B}}

\newcommand{\nomatA}{A}
\newcommand{\nomatB}{Z}
\newcommand{\matA}{\mat \nomatA}
\newcommand{\matB}{\mat \nomatB}
\newcommand{\tmatA}{\mat{\tilde{\nomatA}}}
\newcommand{\tmatB}{\mat{\tilde{\nomatA}}}
\newcommand{\tnomatA}{\tilde{\nomatA}}
\newcommand{\tnomatB}{\tilde{\nomatB}}

%% Stochastics
\newcommand{\stochdom}{\Theta}
\newcommand{\w}{\theta}
\newcommand{\sigfield}{\Sigma}
\newcommand{\pmeasure}{\mathbb P}
\newcommand{\meanval}[1]{\mathbb{E}\left[ {#1} \right]}
\newcommand{\variance}[1]{\mathrm{Var}\left[ {#1} \right]}
\newcommand{\covariance}[1]{\mathrm{Cov}\left[ {#1} \right]}
\newcommand{\covfun}[2]{\Gamma(#1,{#2})}
\newcommand{\pcovfun}[2]{\hat{\Gamma}(#1,{#2})}
\newcommand{\tcovfun}[2]{\tilde\Gamma(#1,{#2})}
\newcommand{\randfield}{\alpha}
\newcommand{\drandfield}[1]{\tilde\alpha_{#1}}
\newcommand{\randvar}{\xi}

%% B-splines
\newcommand{\nsd}{d}
\newcommand{\dom}{\mathcal D}
\newcommand{\pdom}{{\hat{\mathcal{D}}}}
\newcommand{\nelms}{N}
\newcommand{\ndofs}{n}
\newcommand{\physdim}{d}
\newcommand{\paradim}{\physdim}
\newcommand{\p}{p}
\newcommand{\q}{q}
\newcommand{\kntvec}{\Xi}
\newcommand{\bs}{B}



